Storing Encoded Episodes as Concepts for Continual Learning

The two main challenges faced by continual learning approaches are catastrophic forgetting and memory limitations on the storage of data. To cope with these challenges, we propose a novel, cognitively-inspired approach which trains autoencoders with Neural Style Transfer to encode and store images. Reconstructed images from encoded episodes are replayed when training the classifier model on a new task to avoid catastrophic forgetting. The loss function for the reconstructed images is weighted to reduce its effect during classifier training to cope with image degradation. When the system runs out of memory the encoded episodes are converted into centroids and covariance matrices, which are used to generate pseudo-images during classifier training, keeping classifier performance stable with less memory. Our approach increases classification accuracy by 13-17% over state-of-the-art methods on benchmark datasets, while requiring 78% less storage space.

==> realated_work.tex <==
\section{Related Work}
\label{sec:related_work}
In this section we review deep learning techniques specifically designed for class-incremental setting. Most recent approaches to class-incremental learning store a portion of the real images ("episodic memory") belonging to the old classes to avoid catastrophic forgetting when learning new classes \cite{Rebuffi_2017_CVPR,Castro_2018_ECCV}. iCaRL~\cite{Rebuffi_2017_CVPR} combines knowledge distillation~\cite{Hinton15} and the NCM (Nearest Class Mean) classifier to produce a class-incremental classifier. Knowledge distillation uses a distillation loss term that forces the labels of the training data of previously learned classes to remain the same when learning new classes. iCaRL uses real images of old classes while learning a representation for the new classes and uses the NCM classifier for classification of the old and new classes. EEIL~\cite{Castro_2018_ECCV} simply improves upon iCaRL with an end-to-end learning approach using the same ideas of knowledge distillation and the storage of real samples.

To avoid the storage of real samples of the old classes, several techniques use generative networks \cite{Seff17,Shin17,Wu18_NIPS,Ostapenko_2019_CVPR}. These approaches model previous class statistics and regenerate images belonging to the old classes when learning new classes. Both \cite{Shin17} and \cite{Wu18_NIPS} use generative replay in which the generator must be trained on a mixture of generated old class images and real images from the new classes. Unfortunately, this approach causes images belonging to classes learned in earlier increments to start to semantically drift, i.e. the quality of images degrades because of the repeated training on synthesized images. Ostapenko et al.~\cite{Ostapenko_2019_CVPR} avoids semantic drift by training the GAN only once on the data of each class. Catastrophic forgetting is avoided by applying a technique similar to elastic weight consolidation (EWC) \cite{kirkpatrick17} in which changes in important weights needed for old classes are avoided when learning new classes. They also grow their network when it runs out of memory while learning new classes, which can be difficult to apply in situations with restricted memory. One major issue with GAN based approaches is that GANs tend to generate images that do not belong to any of the learned classes which decreases classification accuracy. For these reasons, most approaches only perform well on less complex datasets such as MNIST \cite{Lechun98} but perform poorly on more complex datasets such as CIFAR-10 \cite{Krizhevsky09} and ImageNet \cite{Russakovsky15}. We avoid the problem of generating images that do not belong to any learned class by training autoencoders instead of GANs. To avoid catastrophic forgetting, we store the features (encoded episodes) generated by the autoencoder for old class data.

Comparatively little work has focused on using autoencoders to generate samples because the images generated by autoencoders are blurry (lacking high frequency components) limiting their usefulness for classifier training \cite{hattori14,kemker18}. Hattori \cite{hattori14} and Kemker et al. \cite{kemker18} are two of the few approaches to use autoencoders to encode and store real data, drawing resemblances to the structure of the mammalian hippocampus~\cite{renoult15}. Hattori \cite{hattori14} uses autoencoders on binary pixel images and Kemker et al. \cite{kemker18} uses a network pre-trained on ImageNet to extract the feature embeddings of real images, applying the autoencoder to the feature embeddings. Neither of these approaches are scalable to high-dimensional RGB images. Moreover, the use of a pre-trained network to extract features gives \cite{kemker18} an unfair advantage compared to other approaches. As discussed in Section \ref{sec:autoencoder_training}, we avoid the problem of image blurriness by using ideas from the Neural Style Transfer (NST) algorithm \cite{Gatys_2016_CVPR}. 
